Data Contamination Report from the 2024 CONDA Shared Task

The 1st Workshop on Data Contamination (CONDA 2024) focuses on all relevant aspects of data contamination in natural language processing, where data contamination is understood as situations where evaluation data is included in pre-training corpora used to train large scale models, compromising evaluation results. The workshop fostered a shared task to collect evidence on data contamination in current available datasets and models. The goal of the shared task and associated database is to assist the community in understanding the extent of the problem and to assist researchers in avoiding reporting evaluation results on known contaminated resources. The shared task provides a structured, centralized public database for the collection of contamination evidence, open to contributions from the community via GitHub pool requests. This first compilation paper is based on 566 reported entries over 91 contaminated sources from a total of 23 contributors. The details of the individual contamination events are available in the platform. The platform continues to be online, open to contributions from the community.

==> tables/corpus.tex <==
\begin{table*}[!ht]\centering
    \setlength\belowcaptionskip{-8px}
    \setlength\tabcolsep{3pt}
    \scriptsize
    \rowcolors{1}{}{lightgray} \ra{1.2}
    \resizebox{0.99\linewidth}{!}{
        \begin{tabular}{
            l
            >{\raggedright\arraybackslash}p{10cm}
            }\toprule
            \textbf{Contaminated Source}       & \textbf{Evaluation Set}                                                                                                                                                                                                                                                                                                                                                                               \\\midrule
            allenai/c4                         & sem\_eval\_2014\_task\_1, race, nyu-mll/glue, amazon\_reviews\_multi, liar, reddit\_tifu, stsb\_multi\_mt, wiki\_qa, gigaword, piqa, esnli, scitail, snli, ibm/duorc, math\_qa, swag, wiki\_bio, xnli, allenai/scicite, aeslc, billsum, AMR-to-Text, winograd\_wsc, squadshifts, head\_qa, xsum, health\_fact, EdinburghNLP/xsum, UCLNLP/adversarial\_qa, paws, sick, super\_glue, paws-x, scan, lama \\
            CommonCrawl                        & allenai/ai2\_arc, tau/commonsense\_qa, ceval/ceval-exam, cais/mmlu, Rowan/hellaswag, winogrande                                                                                                                                                                                                                                                                                                       \\
            EleutherAI/pile                    & sem\_eval\_2014\_task\_1, nyu-mll/glue, amazon\_reviews\_multi, mbpp, openai\_humaneval, liar, stsb\_multi\_mt, wiki\_qa, gigaword, piqa, esnli, scitail, snli, ibm/duorc, swag, xnli, allenai/scicite, aeslc, billsum, winograd\_wsc, squadshifts, head\_qa, xsum, health\_fact, UCLNLP/adversarial\_qa, paws, sick, super\_glue, paws-x, scan                                                       \\
            oscar-corpus/OSCAR-2301            & sem\_eval\_2014\_task\_1, crows\_pairs, nyu-mll/glue, race, amazon\_reviews\_multi, openai\_humaneval, liar, stsb\_multi\_mt, wiki\_qa, gigaword, piqa, esnli, scitail, snli, math\_qa, swag, xnli, allenai/scicite, aeslc, billsum, winograd\_wsc, squadshifts, head\_qa, xsum, health\_fact, UCLNLP/adversarial\_qa, paws, sick, super\_glue                                                        \\
            togethercomputer/RedPajama-Data-V2 & sem\_eval\_2014\_task\_1, race, nyu-mll/glue, amazon\_reviews\_multi, liar, stsb\_multi\_mt, wiki\_qa, gigaword, piqa, esnli, scitail, snli, ibm/duorc, math\_qa, swag, xnli, allenai/scicite, aeslc, billsum, winograd\_wsc, squadshifts, head\_qa, xsum, health\_fact, UCLNLP/adversarial\_qa, mc\_taco, paws, samsum, sick, super\_glue, paws-x, scan                                              \\
            bigscience/xP3                     & facebook/flores                                                                                                                                                                                                                                                                                                                                                                                       \\
            EleutherAI/proof-pile-2            & gsm8k, hendrycks/competition\_math                                                                                                                                                                                                                                                                                                                                                                    \\
            bigcode/the-stack                  & openai\_humaneval, mbpp                                                                                                                                                                                                                                                                                                                                                                               \\
            \bottomrule
        \end{tabular}
    }
    \caption{A summary of the \textit{dev} or \textit{test} sets found at above 0\% contamination in each training corpus.}\label{tab:report-corpora}
\end{table*}

==> tables/model.tex <==

\begin{table*}[!t]\centering
    \setlength\belowcaptionskip{-8px}
    \setlength\tabcolsep{3pt}
    \scriptsize
    \rowcolors{1}{}{lightgray} \ra{1.2}
    \resizebox{0.99\linewidth}{!}{
        \begin{tabular}{
            l
            >{\raggedright\arraybackslash}p{10cm}
            }\toprule
            \textbf{Contaminated Source} & \textbf{Evaluation Set}                                                                                                                                                                                                                                                                                                                                                                    \\\midrule
            GPT-3                        & Reversed Words, race, quac, Anagrams 1, Cycled Letters, mandarjoshi/trivia\_qa, ibragim-bad/arc\_easy, SAT Analogies, piqa, Rowan/hellaswag, wmt/wmt16, stanfordnlp/coqa, cimec/lambada, natural\_questions, winograd\_wsc, ucinlp/drop, rmanluo/RoG-webqsp, rajpurkar/squad\_v2, allenai/openbookqa, Symbol Insertion, Anagrams 2, super\_glue, ibragim-bad/arc\_challenge, facebook/anli \\
            GPT-3.5                      & samsum, yelp\_review\_full, imdb, ag\_news, nyu-mll/glue, conll2003, winogrande, rajpurkar/squad\_v2, cais/mmlu, EdinburghNLP/xsum, allenai/openbookqa, xlangai/spider, truthful\_qa                                                                                                                                                                                                       \\
            GPT-4                        & samsum, yelp\_review\_full, gsm8k, imdb, ibragim-bad/arc\_challenge, nyu-mll/glue, ucinlp/drop, winogrande, openai\_humaneval, ag\_news, EdinburghNLP/xsum, cais/mmlu, Rowan/hellaswag, allenai/openbookqa, truthful\_qa, bigbench                                                                                                                                                         \\
            PaLM 2                       & EdinburghNLP/xsum, csebuetnlp/xlsum, wiki\_lingua                                                                                                                                                                                                                                                                                                                                          \\
            GPT-3.5-turbo                & openai\_humaneval, HumanEval\_R                                                                                                                                                                                                                                                                                                                                                            \\
            FLAN                         & natural\_questions, mandarjoshi/trivia\_qa, story\_cloze, piqa, super\_glue, ibragim-bad/arc\_challenge, ucinlp/drop, rajpurkar/squad\_v2, ibragim-bad/arc\_easy, Rowan/hellaswag, allenai/openbookqa, facebook/anli, winogrande, wmt/wmt16                                                                                                                                                \\
            GLaM                         & stanfordnlp/coqa, natural\_questions, mandarjoshi/trivia\_qa, story\_cloze, cimec/lambada, piqa, super\_glue, ibragim-bad/arc\_challenge, race, quac, winograd\_wsc, rajpurkar/squad\_v2, ibragim-bad/arc\_easy, Rowan/hellaswag, allenai/openbookqa, facebook/anli, winogrande                                                                                                            \\
            LLaMa 2-13B                  & allenai/openbookqa, winogrande, truthful\_qa                                                                                                                                                                                                                                                                                                                                               \\
            Mistral-7B                   & allenai/openbookqa, winogrande, truthful\_qa, cais/mmlu                                                                                                                                                                                                                                                                                                                                    \\
            PaLM                         & cimec/lambada, super\_glue, ibragim-bad/arc\_challenge, winograd\_wsc, rmanluo/RoG-webqsp, rajpurkar/squad\_v2, mandarjoshi/trivia\_qa, ibragim-bad/arc\_easy                                                                                                                                                                                                                              \\
            Claude 3 Opus                & facebook/flores                                                                                                                                                                                                                                                                                                                                                                            \\
            bigscience/bloomz-*            & facebook/flores                                                                                                                                                                                                                                                                                                                                                                            \\

            bigscience/mt0-*          & facebook/flores                                                                                                                                                                                                                                                                                                                                                                            \\

            BAAI/Aquila2-34B             & gsm8k, hendrycks/competition\_math                                                                                                                                                                                                                                                                                                                                                         \\
            BAAI/AquilaChat2-34B         & gsm8k                                                                                                                                                                                                                                                                                                                                                                                      \\
            EleutherAI/llemma\_*       & gsm8k, hendrycks/competition\_math                                                                                                                                                                                                                                                                                                                                                         \\

            Qwen/Qwen-1\_8B              & gsm8k, hendrycks/competition\_math                                                                                                                                                                                                                                                                                                                                                         \\
            BAAI/Aquila2-7B              & hendrycks/competition\_math                                                                                                                                                                                                                                                                                                                                                                \\
            Qwen/Qwen-*                & hendrycks/competition\_math                                                                                                                                                                                                                                                                                                                                                                \\
                                                                                        
            THUDM/chatglm3-6b            & hendrycks/competition\_math                                                                                                                                                                                                                                                                                                                                                                \\
            internlm/internlm2-*        & hendrycks/competition\_math                                                                                                                                                                                                                                                                                                                                                                \\

            mistralai/Mistral-7B-v0.1    & ibragim-bad/arc\_easy                                                                                                                                                                                                                                                                                                                                                                      \\
            \bottomrule
        \end{tabular}
    }
    \caption{A summary of the \textit{dev} or \textit{test} sets found at above 0\% contamination in each reported model. The "*" is used to indicate the different versions or sizes of the models.}
    \label{tab:report-models}
\end{table*}

